Time Advances and Dispersive Constraints in Dressed Gravitational Scattering

We derive a low energy group time advance in 4D dressed gravitational scattering at leading eikonal order with full soft dependence for a sharp dressing profile of finite soft scale. Dispersive matching of nonnegative absorption excludes the amplitude's analytic crossing with high energy boundedness. This reflects internal scales growing with energy via string diffusion in quantum gravity and high energy nonlinear graviton rescattering, coupled to soft clouds beyond leading soft order. Interference preserving joint detection of hard particles and coherent soft radiation may reveal the advance.

==> supplement_references.tex <==
%
%
%
%
%
%
%
%
\begin{thebibliography}{9}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{https://doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%
\bibitem [{\citenamefont {Arkani-Hamed}\ \emph {et~al.}(2021)\citenamefont
  {Arkani-Hamed}, \citenamefont {Pate}, \citenamefont {Raclariu},\ and\
  \citenamefont {Strominger}}]{sm-Arkani-Hamed:2020gyp}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Arkani-Hamed}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Pate}},
  \bibinfo {author} {\bibfnamefont {A.-M.}\ \bibnamefont {Raclariu}},\ and\
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Strominger}},\ }\bibfield
   {title} {\bibinfo {title} {{Celestial amplitudes from UV to IR}},\ }\href
  {https://doi.org/10.1007/JHEP08(2021)062} {\bibfield  {journal} {\bibinfo
  {journal} {JHEP}\ }\textbf {\bibinfo {volume} {08}}\bibfield  {number}
  {\bibinfo  {number} { (2021)},\ \bibinfo {pages} {062}},\ }\Eprint
  {https://arxiv.org/abs/2012.04208} {arXiv:2012.04208 [hep-th]} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Ware}\ \emph {et~al.}(2013)\citenamefont {Ware},
  \citenamefont {Saotome},\ and\ \citenamefont {Akhoury}}]{sm-Ware:2013zja}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Ware}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Saotome}},\ and\
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Akhoury}},\ }\bibfield
  {title} {\bibinfo {title} {{Construction of an asymptotic S matrix for
  perturbative quantum gravity}},\ }\href
  {https://doi.org/10.1007/JHEP10(2013)159} {\bibfield  {journal} {\bibinfo
  {journal} {JHEP}\ }\textbf {\bibinfo {volume} {10}}\bibfield  {number}
  {\bibinfo  {number} { (2013)},\ \bibinfo {pages} {159}},\ }\Eprint
  {https://arxiv.org/abs/1308.6285} {arXiv:1308.6285 [hep-th]} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Hannesdottir}\ and\ \citenamefont
  {Schwartz}(2020)}]{sm-HannesdottirSchwartz:2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Hannesdottir}}\ and\ \bibinfo {author} {\bibfnamefont {M.~D.}\ \bibnamefont
  {Schwartz}},\ }\bibfield  {title} {\bibinfo {title} {{$S$ -Matrix for
  massless particles}},\ }\href {https://doi.org/10.1103/PhysRevD.101.105001}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo
  {volume} {101}},\ \bibinfo {pages} {105001} (\bibinfo {year} {2020})},\
  \Eprint {https://arxiv.org/abs/1911.06821} {arXiv:1911.06821 [hep-th]}
  \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Choi}\ and\ \citenamefont
  {Akhoury}(2018)}]{sm-Choi:2017ylo}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Choi}}\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Akhoury}},\
  }\bibfield  {title} {\bibinfo {title} {{BMS Supertranslation Symmetry Implies
  Faddeev-Kulish Amplitudes}},\ }\href
  {https://doi.org/10.1007/JHEP02(2018)171} {\bibfield  {journal} {\bibinfo
  {journal} {JHEP}\ }\textbf {\bibinfo {volume} {02}}\bibfield  {number}
  {\bibinfo  {number} { (2018)},\ \bibinfo {pages} {171}},\ }\Eprint
  {https://arxiv.org/abs/1712.04551} {arXiv:1712.04551 [hep-th]} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Cachazo}\ and\ \citenamefont
  {Strominger}(2014)}]{sm-CachazoStrominger:2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Cachazo}}\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Strominger}},\ }\href@noop {} {\bibinfo {title} {{Evidence for a New Soft
  Graviton Theorem}}} (\bibinfo {year} {2014}),\ \Eprint
  {https://arxiv.org/abs/1404.4091} {arXiv:1404.4091 [hep-th]} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Sen}(2017)}]{sm-Sen:2017soft}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Sen}},\ }\bibfield  {title} {\bibinfo {title} {{Soft Theorems in Superstring
  Theory}},\ }\href {https://doi.org/10.1007/JHEP06(2017)113} {\bibfield
  {journal} {\bibinfo  {journal} {JHEP}\ }\textbf {\bibinfo {volume}
  {06}}\bibfield  {number} {\bibinfo  {number} { (2017)},\ \bibinfo {pages}
  {113}},\ }\Eprint {https://arxiv.org/abs/1702.03934} {arXiv:1702.03934
  [hep-th]} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sahoo}\ and\ \citenamefont
  {Sen}(2019)}]{sm-Sahoo:2018lxl}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Sahoo}}\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Sen}},\
  }\bibfield  {title} {\bibinfo {title} {{Classical and Quantum Results on
  Logarithmic Terms in the Soft Theorem in Four Dimensions}},\ }\href
  {https://doi.org/10.1007/JHEP02(2019)086} {\bibfield  {journal} {\bibinfo
  {journal} {JHEP}\ }\textbf {\bibinfo {volume} {02}}\bibfield  {number}
  {\bibinfo  {number} { (2019)},\ \bibinfo {pages} {086}},\ }\Eprint
  {https://arxiv.org/abs/1808.03288} {arXiv:1808.03288 [hep-th]} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Ciafaloni}\ \emph {et~al.}(2016)\citenamefont
  {Ciafaloni}, \citenamefont {Colferai}, \citenamefont {Coradeschi},\ and\
  \citenamefont {Veneziano}}]{sm-Ciafaloni:2015unified}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Ciafaloni}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Colferai}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Coradeschi}},\ and\
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Veneziano}},\ }\bibfield
  {title} {\bibinfo {title} {{Unified limiting form of graviton radiation at
  extreme energies}},\ }\href {https://doi.org/10.1103/PhysRevD.93.044052}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo
  {volume} {93}},\ \bibinfo {pages} {044052} (\bibinfo {year} {2016})},\
  \Eprint {https://arxiv.org/abs/1512.00281} {arXiv:1512.00281 [hep-th]}
  \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ciafaloni}\ \emph {et~al.}(2019)\citenamefont
  {Ciafaloni}, \citenamefont {Colferai},\ and\ \citenamefont
  {Veneziano}}]{sm-Ciafaloni:2019infrared}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Ciafaloni}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Colferai}},\ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Veneziano}},\ }\bibfield  {title} {\bibinfo {title} {{Infrared features of
  gravitational scattering and radiation in the eikonal approach}},\ }\href
  {https://doi.org/10.1103/PhysRevD.99.066008} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo
  {pages} {066008} (\bibinfo {year} {2019})},\ \Eprint
  {https://arxiv.org/abs/1812.08137} {arXiv:1812.08137 [hep-th]} \BibitemShut
  {NoStop}%
\end{thebibliography}%

